CoderEval: A Benchmark of Pragmatic Code Generation with Generative Pre-trained Models

Code generation models based on the pre-training and fine-tuning paradigm have been increasingly attempted by both academia and industry, resulting in well-known industrial models such as Codex, CodeGen, and PanGu-Coder. To evaluate the effectiveness of these models, multiple existing benchmarks are proposed, including only cases of generating a standalone function, i.e., a function that may invoke or access only built-in functions and standard libraries. However, non-standalone functions, which typically are not included in the existing benchmarks, constitute more than 70% of the functions in popular open-source projects, and evaluating models' effectiveness on standalone functions cannot reflect these models' effectiveness on pragmatic code generation scenarios. To help bridge the preceding gap, in this paper, we propose a benchmark named CoderEval, consisting of 230 Python and 230 Java code generation tasks carefully curated from popular real-world open-source projects and a self-contained execution platform to automatically assess the functional correctness of generated code. CoderEval supports code generation tasks from six levels of context dependency, where context refers to code elements such as types, APIs, variables, and consts defined outside the function under generation but within the dependent third-party libraries, current class, file, or project. CoderEval can be used to evaluate the effectiveness of models in generating code beyond only standalone functions. By evaluating three code generation models on CoderEval, we find that the effectiveness of these models in generating standalone functions is substantially higher than that in generating non-standalone functions. Our analysis highlights the current progress and pinpoints future directions to further improve a model's effectiveness by leveraging contextual information for pragmatic code generation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> approach/benchmark.tex <==
\subsection{Benchmark: \wenwangbench{}}
\label{sec: benchmark}

In this section, we introduce a pragmatic benchmark of code generation named \wenwangbench{}.
We first introduce the construction of \wenwangbench{}, followed by the workflow of a verification platform for automatic evaluation.

\subsubsection{Benchmark Construction}

We construct the benchmark from recently-committed code on GitHub.
First, we sort all projects with successfully-executed CI by the number of stargazers descendingly and keep the top 1,000 projects with at least one new commit since January 1, 2022.
Next, we extract all collected functions in these projects from the database, then kept the ones that meet all the following conditions:

\begin{itemize}
    \item does not exist in \wenwangdataset{}
    \item is not a test or deprecated function
    \item with a function-level docstring in English
    \item with at least three lines of code in the function body
    \item with at least one test case collected during the CI execution, and the input\&output can be successfully deserialized with the \emph{dill} library
    \item can run successfully in the verification platform and passed the test cases
\end{itemize}

We adopt a series of works to improve the confidence and reliability of the benchmark.
For the collected functions, we remove them from the dataset, search in the dataset again using the docstring and function signature, and remove \emph{all} matched samples to ensure that there is no overlap between the benchmark and the dataset.
To simulate the practical scenario, we classify each collected function to a runnable level with the same approach in Section~\ref{sec.classify}, and control the proportion of each level for a similar distribution with the dataset.
% To reduce false positives during evaluation, for problems with only one test case, we manually mutated the input and ran the function to get the expected output through the verification platform, and appended the input/output pairs as the supplementary test cases.
When verifying the correctness of a function generated by models, our verification platform adds the $main$ function to the file to which the function belongs and runs the file. 
The input and output of test cases obtained through CI are run in the entire project environment. 
Therefore, to ensure that the verification platform can correctly verify the function generated by the model, we execute test cases separately at the file level and use the output as the output of the test cases in the benchmark.

Finally, we involve 230 functions from 43 projects in \wenwangbench{}.
The right part of Figure~\ref{fig.run_dep_res} shows the distribution of runnable levels on \wenwangbench{}.
Besides the internal, contextual, and meta information, each function also contains supplementary test cases. The average number of test cases for each function in \wenwangbench{} is 10.34, and more than 73\% of functions have more than one test case in the benchmark.

% Even though the average test case for each function is not low, there are some functions with only 1 or 2 test cases. 
% In the future, we will try to supplement more than five test cases for each function in \wenwangbench{}.
% According to the functions in the newly submitted files after January 1, 2022 based on commit\_time, we obtained a total of 152 open source projects configured with Tox CI. A total of 8700 newly submitted functions were obtained from these open source projects, of which 5429 were functions with docstring. 
% Our criterion for judging whether a function is a newly submitted function is based on the module + function signature as the unique identifier.
% The data items we collected in our benchmark totally contains docstring and test cases collected by CI. 
% To expand the number of functions in our benchmark, we also collected 140 functions in the newly submitted files after January 1, 2022 based on commit\_time, these 140 functions contain docstring, but do not contain test cases. 
% Since the benchmark requires supporting test cases, For functions without test cases, we use copilot to generate test cases for the functions. Then one of our author check the test cases generated by copilot manually and finally expand 36 functions.

% To make our benchmark can validate the function with multiple runnable level, we also classify the data in our benchmark into six runnable level: self\_contained, slib\_runnable, plib\_runnable, class\_runnable, file\_runnable, and others.
% We use the same technique of runnable classification for \wenwangdataset{} to classify the runnable level of a function in the \wenwangbench{}.
% We find the distribution runnable classification of \wenwangbench{} is similar with \wenwangdataset{}.


\subsubsection{Verification Platform}

Since \wenwangbench{} involves functions with contextual dependency and non-primitive types, we need a verification platform to provide a ready runtime environment to automatically run and verify the code generated by code generation models.

We base this platform on Docker, where we clone and set up environments for all 43 projects.
To avoid Python and library version conflicts, under each repository's root directory, we first use \emph{pyenv} to set the local Python version to the highest version specified in the CI configuration, then use \emph{venv} to create an individual virtual environment for the current project.
After that, we trigger the CI tool to install dependencies and set up the project before running tests.

With the environment ready and given a model to evaluate, the platform can automatically inject the solution it generates into the project code and invokes the function to compare the actual output with the expected output.
To invoke the target function correctly, we generate the entry point code to set up some necessary prerequisites (like initializing the object before calling a member function) and load the input/output data into memory via deserialization.
Given \emph{n} solutions generated by the model, the platform automatically replaces the original function with each of them to \emph{simulate} how the code generation and recommendation work in an actual IDE.
After the replacement, the entry point code will be started, and the running output (e.g., return values, exceptions, errors, and console output) will be captured.
If the function returns with no error and exception, the platform will compare the actual output with the expected output. Comparison results of all 230 tasks will be used to compute the Pass@K metric at the end of the evaluation.


% Compared with HumanEval, \wenwangbench{} has two main advantages: (1) The test object for \wenwangbench{} is the functions in realistic development scenarios, and the functions in \wenwangbench{} are mined from open source projects. (2) \wenwangbench{} not only supports functions that are valid for the object with basic type (e.g., int, float, str), but also supports the object with complex types. The functions with complex objects often belong to class-level, file-level and project-level runnable.
% To achieve the first advantage, we strictly mine functions that not appear in \wenwangdataset{}, and most of them are submitted after 2022 from GitHub, and use CI to collect their test cases.
% Since the object in functions in HumanEval's are basic types, it does not need to consider the validation of functions belong to class, file, and project-level. 
% To achieve the second advantage, we built a verification platform that supports class, file, and project level. Next, we will introduce the construction of \wenwangbench{}'s verification platform in detail.
% To achieve the accuracy of the functions for verifying class-level dependencies, file-level dependencies, and project-level dependencies, we first need to serialize the input and output as objects of complex types and store them in the database in binary form. These stored data are then deserialized from the database into objects that can be executed in the program when testing functions that rely on objects of complex types. It is easy to serialize objects of complex types while the project is running, because all elements of serialization dependencies are available in the currently running project. At the same time, this requires that when deserializing the data stored in the database, it also needs to be executed in the entire project. Therefore, when verifying the correctness of functions in \wenwangbench{}, the verification platform of \wenwangbench{} needs the entire project where the function is located as the context.
% In the end, we selected 43 projects with a total of 230 functions for \wenwangbench{}.



% To verify the correctness of the functions in \wenwangbench{}, we need to automatically generate the correct calling function for each function. It should be noted that the calling function of dependent class-level executable functions is written inconsistently with other levels. Because the class level first instantiates the object of the class and other levels don't need to. 
% %Figures x and y show how calling functions are written at the class level and other levels.

% deserialize input and output of test cases, run and get, compare with

% Changed relative references in python files to absolute references
% Since there are relative references in the python file, the file cannot be run directly. And a large number of functions in our benchmark appear in python files where relative references exist. Therefore, we automatically change the relative reference in python to absolute reference.

% For each generated code to be tested, we replace the function location (in a file in a project) with the code in a python-compilable and executable format.
% Then execute the code in the project and determine whether the code is generated correctly according to whether the test cases are passed.


==> approach/dataset.tex <==
\subsection{Dataset: \wenwangdataset}
\label{sec: dataset}

In this section, we introduce the detailed construction of \wenwangdataset{}, including the selection of open-source projects, data collection, and further analysis.

\subsubsection{Project Selection}

Following the Codex's way of collecting open-source data, we consider Python3-compatible GitHub repositories using Travis\footnote{\url{https://www.travis-ci.com/}} or Tox\footnote{\url{https://tox.wiki/en/latest/}} as the continuous integration (CI) system, which are the most popular CI tools for Python.
Specifically, we first search on GitHub for repositories with Python as the first primary programming language, then check whether there existing the configuration file (travis.y(a)ml, tox.ini) under the repository root to determine whether this project uses Travis or Tox. For projects that use Travis and Tox, we further open the configuration file and check the target Python version specified for testing to determine whether this project supports Python version 3.
Finally, as shown in Figure~\ref{fig: distribution_travis_tox}, by June of 2022, we collect a total of 136,446 repositories, 36,039 of which configures Travis and Tox at the same time.

\begin{figure}
	\centering
	\includegraphics[width=0.2\textwidth]{figure/travis_tox.pdf}
	\caption{Distribution of Travis and Tox Projects}
	\label{fig: distribution_travis_tox}
  \vspace*{-1ex}
\end{figure}

\subsubsection{Data Collection}

For each selected project, we try to rerun the CI locally and collect the functions invoked during a successful CI execution as our dataset.
Similar to Codex, we consider these functions to be correctly implemented since they are directly or indirectly tested by the developer.
For each function, we collect the following information for later use:

\begin{itemize}
    \item Internal Info: the annotation, docstring, signature, and code snippet of the function
    % \item Contextual Info: the content of the source file in which the function resides, the input argument values and the output/return values (if exists). For data of non-primitive types, we used the \textit{dill} library to serialize the object in binary format
    \item Contextual Info: the content of the source file in which the function resides
    \item Meta Info: the location (project, file path, and line ranges) of the function, and the version control information (commit id, commit timestamp, and committer) of the most recent commit that touched the function
\end{itemize}

To efficiently collect data from a massive number of projects, there are three challenges: (1) automatically prepare the environment required by the CI tool and the project, (2) efficiently analyze such a massive number of projects, and (3) dynamically collect the above information during testing.
We tackle these challenges step by step: First, based on the Ubuntu+Travis docker image from DockerHub, we prepare a base environment and wrote a system to automatically clone the repository with \textit{Git}, install the correct Python version configured by the CI tool with \textit{pyenv}.
After installing the Python interpreter, the system injects a tracing function into the installed Python, which would capture and save the above information into a MongoDB database when running Python code from the project. Next, we deploy this docker image to 500 containers on a cloud computing cluster with \textit{Kubernates} and trigger the system to continuously analyze the next project in a queue of tasks. In this way, we are able to analyze all projects parallelly in 350 hours.

To make \wenwangdataset{} more useful for generating non-standalone functions, we also provide oracle\_contextual and all\_contextual information for \wenwangdataset{}.
\emph{oracle\_context} information can be used as part of the input to the model in the inference stage, to verify whether prompting the model with the oracle information can improve the performance. However, it is usually difficult for the model to know oracle information in advance, so \wenwangdataset{} also provides the \emph{all\_context} information, that is, all types, variables, and APIs defined/imported in the current file. 
\wenwangdataset{} can be used by the model in both the training and inference stage.

In total, we collected 300,000 functions from all projects and filtered out those without a valid docstring, resulting in 103,541 functions as the final dataset.
Compared with Codex's dataset, we do not restrict the standalone functions or use a pre-trained model to filter the data to avoid bias in distribution and tight binding with specific models.
Besides, we additionally consider functions without output/return value and functions that involve data of user-defined types in the input/output.
Therefore, we believe it provides a more reasonable choice when fine-tuning pre-trained models towards the task of generating code beyond standalone functions.



% Similar with CoderEval, we also do several data augmentations for each function in 
% \subsubsection{Data Augmentation}
% \label{sec.classify}

% To better understand the task of pragmatic code generation, we additionally classify the dataset into different \textit{runnable levels} according to the \textit{contextual dependency} of functions.


% \paragraph{Contextual Dependency Identification}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \begin{table*}[t]
% \caption{Contextual Dependency Types}
%     \centering
%     \footnotesize
%     \renewcommand{\arraystretch}{1.5}
%     \vspace*{-1.5ex}
%     \begin{tabular}{llll}
%     \toprule
%     Database Schema & \multicolumn{1}{c}{Dependency Type} & \multicolumn{1}{c}{Explanation} & \multicolumn{1}{c}{Example} \\ 
%     \midrule
%     \multirow{6}{*}{\makecell[l]{dependency: \{ \\
%     \hspace{\parindent} builtin: boolean, \\
%     \hspace{\parindent} standard\_lib: boolean, \\
%     \hspace{\parindent} public\_lib: boolean, \\
%     \hspace{\parindent} current\_class: boolean, \\
%     \hspace{\parindent} current\_file: boolean, \\
%     \hspace{\parindent} current\_project: boolean  \\
% \} }} & builtin & Python builtin types and functions, no need to import. & min(), round(), print() \\
%      & standard\_lib & Python standard libraries/modules, no need to install. & os, subprocess, sys \\
%      & public\_lib & Publicly available libraries on pypi.org, pip install first. & unittest2, requests, urllib \\
%      & current\_class & Code outside the function but inside the parent class. & self.xxx, self.f(), X.f() \\
%      & current\_file & Code outside the parent class but inside the current file. & func(), URL, name \\
%      & current\_project & Code in the other source files of the current project. & superclass (defined in anther file) \\
%      \bottomrule
%     \end{tabular}
    
%     \label{tab: run_dep_cla}
% \end{table*}
% We denote the context code elements that a function directly requires to run as its contextual dependency, which includes language-builtins, standard libraries, third-party public libraries, and code outside the function but within the current class, file, or project.
% Table~\ref{tab: run_dep_cla} shows the definition and exemplary explanation for each dependency type in Python code.
% For each entry in the database, we use a field named \textit{dependency} to store the identified dependencies.





% % Figure~\ref{fig: run_dep_imp} shows how we identified the contextual dependency of a function through program analysis on the whole project.
% We identify the contextual dependency of a function through program analysis on the whole project.
% Before the analysis, we first need to build a knowledge base that helps distinguish the references of Python-builtins, and the imports of standard or public libraries from the project-specific code.
% To do this, we cache all built-in types/functions/variables/constants and standard library names for each Python version from 3.0.0 to 3.10.0, as well as all public-available libraries on pypi.org.
% With this knowledge base, given a function to analyze, we retrieve the database to get the source file that it came from, then parse it to get a list of defined types/functions/variables/constants.
% For each dependency type, the criterion for setting it to true was whether the function \textit{used} the code of this type.
% For example, for a member function in a class, if it invokes a builtin function \lstinline{sorted()} to manipulate a member variable \lstinline{self.x}, we set the \lstinline{builtin} and \lstinline{current_class} to true.

% % \begin{figure*}
% % 	\centering
% % 	\includegraphics[width=0.7\textwidth]{figure/runnable_classifcation.png}
% % 	\caption{The Overview of Runtime Dependency Classification}
% % 	\label{fig: run_dep_imp}
% % \end{figure*}


% \paragraph{Runnable-level Classification}
% \begin{table}[t]
% \begin{threeparttable}
%     \centering
%     \setlength\tabcolsep{1.1pt}
%     \footnotesize
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Matrix to Classify Runnable Level by Dependency}
%     \vspace*{-1.5ex}
%     \label{tab: run_dep_rdc}
%     \begin{tabular}{@{} ccccccccc @{}} % suppress vertical whitespace at start and end
%         \toprule
%         \diagbox[width=\dimexpr \textwidth/6+2\tabcolsep\relax, height=0.8cm]{ Runnable Level }{Dependency}
%         & \makecell{language \\ builtin} & \makecell{standard \\ library} & \makecell{public \\ library} & \makecell{current \\ class} & \makecell{current \\ file} & \makecell{current \\ project} \\
%         \midrule
%         self\_contained & $\bigcirc$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         slib\_runnable & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         plib\_runnable & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
%         \midrule
%         class\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ & $\times$ \\
%         \midrule
%         file\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ & $\times$ \\
%         \midrule
%         project\_runnable & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\bigcirc$ & $\checkmark$ \\
%         \bottomrule
%     \end{tabular}
%     \emph{\footnotesize
%         $\checkmark$ means true, $\times$ means false, and $\bigcirc$ means true/false.
%     }
%     \vspace*{-2.5ex}
%     \end{threeparttable}
% \end{table}
% According to the identified dependency, we classify the data into six levels, each of which indicates the minimal context scope that a function requires to run.
% The motivation is to simulate different scenarios of pragmatic code generation, analyze the advantage and shortcomings of existing models in more detail, and optimize them more systematically.


% We define a \textit{Dependency Matrix} for the classification, as shown in Table~\ref{tab: run_dep_rdc}.
% In this matrix, the row represents the runnable level, the column represents the dependency type, and each cell indicates whether the level of the row could depend on the dependency type of the column.
% From top to bottom, we define six levels from self\_contained to project\_runnable. Each level indicates the \emph{minimal} context scope a function requires to run.
% For example, plib\_runnable means the function \emph{at most} depends on public libraries,so it can run successfully outside the current source file and project, as long as the required Python version is satisfied and the libraries are installed.
% Note that we determine the runnable level by what it \emph{cannot} depend on, so the higher level wraps the lower levels (see Figure~\ref{fig.run_dep_res}), because intuitively if a function of the lower level can within its scope (say with standard library imports), it can also run given a larger scope (say the current file).



% The left part of Figure~\ref{fig.run_dep_res} shows the distribution of runnable levels on \wenwangdataset{}.
% Most (84\%) of the collected functions are file\_runnable, which indicates that the context information in the current file is necessary and critical for a code generation model to generate the function correctly.
% The class\_runnable functions account for half (54\%) of all functions, which is not surprising considering the prevalence of object-oriented programming in realistic and non-trivial projects.
% On the contrary, slib\_runnable only accounts for 17\% in our dataset but 100\% in the Codex dataset and the HumanEval benchmark. This fact proves the bias and mismatching in the model optimization and evaluation process with HumanEval, especially in the pragmatic generation of code in realistic settings.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figure/dis.pdf}
% 	\caption{Distribution of Runnable Level Classification}
% 	\label{fig.run_dep_res}
% \end{figure}


% --------------------------BACKUPS--------------------------

% First, we reproduced the CI environment of each project locally in docker instances, then injected a tracing function in the environment, which would capture the input, output, invocation location, and context code for each function invoked during integration testing. After that, the CI script was triggered and the data of invoked functions were recorded into a database. We further clustered the collected data into 4 groups, according to the external contextual information (dependencies) that a function requires to run. That is, functions depending on Python-builtin objects, Python-standard libraries, Pypi-public libraries, and the class. We expect this variety could enable the generation of different function types, e.g., self-contained, module, member or class functions. After filtering for maximum model input length, 49K examples are retained for fine-tuning.



% To implement the technique of runtime dependency classification, we first record all python build\_in type functions (e.g., $open$, $sorted$ ...), these functions can be executed directly in the python environment without any import.
% Then we record all the standard libraries in python (e.g., $os$, $subprocess$, $sys$), the functions belong to the standard libraries can directly import the library in the python environment and be executed successfully.
% Next we record the public libraries (e.g., $numpy$, $tensorflow$, $torch$) in python according to the download frequency. 
% Functions belong to the public libraries need to pip install the public library and import the public library in the python environment to execute successfully.
% After completing the above pre-recording, we analyze the dependencies of each level.
% Specifically, given any function to be classified and its file, we first analyze all functions and variables defined in the class or file where the function to be classified belong to.
% % After the preceding analysis, we get  
% Then we perform six dependency level analysis: Python Buildins, StandardLib, PublicLib, Class, File, and Project.



% \subsubsection{Competitive Programming Data}
% The following two datasets often provide dozens of successful code completions for each problem. Therefore, we can upsample each dataset by pairing up to five solutions with each problem description to avail the model of different correct solutions for the same problem specification. APPS~\cite{hendycks-etal-2021-apps} was proposed to benchmark the programming capability of code-generating models. It includes 10,000 programming tasks (5,000 train, 5,000 test) that require code generation/completion given a detailed problem description\footnote{\url{https://github.com/hendrycks/apps}}. Program arguments are provided from standard input as well as function calls, sometimes embedded inside the class. We use the train and test set programs, which we filter for the maximum input length of the model (1,024), retaining 43K examples. Code Contests (CC) is a similar dataset~\cite{alpha_code} for training and evaluation of competition-level code generation\footnote{\url{https://github.com/deepmind/code_contests}}, containing over 13K programming problems. After upsampling and length filtering, we retain 18K instances for fine-tuning.


% To build a dataset suitable for multiple application scenarios (such as competitive programming, realistic development), we construct the \wenwangdataset{} with multiple runnable level.
% To construct the \wenwangdataset{} with multiple runnable level, we first make a runtime dependency classification for each function in the \wenwangdataset{}. 
% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.7\textwidth]{figure/runnable_classify.png}
% 	\caption{Runtime Dependency Classification}
% 	\label{fig: run_dep_cla}
% \end{figure*}

% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.7\textwidth]{figure/runnable_count.png}
% 	\caption{Runnable Classification}
% 	\label{fig: run_dep_rdc}
% \end{figure*}
% We further clustered the collected data into 4 groups, according to the external contextual information (dependencies) that a function requires to run. That is, functions depending on the Python-builtin objects, the Python-standard libraries, the Pypi-public libraries, and the  class. We expect this variety would enable the generation of different function types, e.g., self-contained, module, member or class functions. After filtering for maximum model input length, 49K examples are retained for fine-tuning.

% \subsection{Sub-Runnable Open Source Data}

% After analyzing the previous part of the data, we found that in solving the competitive programs, using self\_contained, slib\_runnable, and plib\_runnable level data for finetune is the best. In this section, we analyze all self\_contained and slib\_runnable functions with docstring on GitHub, collecting a total of 1 million functions


% The file\_runnable level accounts for the largest proportion in open source projects, which is about 30\%. The second-highest percentage is the class\_runnable level, which accounts for 28\%. The slib\_runnable level accounts for only 6\%. 
% In addition, we can find that the first three types (i.e., self\_contained, slib\_runnable, and plib\_runnable) account for only 26\%. That is, the existing benchmark can only test about 26\% of the data in open source projects. 
% This ratio is far from sufficient. Therefore, the benchmark (\wenwangbench{}) for realistic development scenarios is provided later in this paper to alleviate this issue.

==> approach/model.tex <==
\subsection{Model: \wenwangcoder{}}
\label{sec: wenwang}


In this section, we introduce \wenwangcoder{}, a model fine-tuned on \codePLM{} using the \wenwangdataset{} with a \technique{} fine-tuning technique to improve the code generation capability of a pre-trained model on generating the code beyond standalone functions.
%The key idea is to fine-tune the pre-trained model with contextual information, to enhance its awareness of the context when generating code in practice.

The motivation behind our \technique{} fine-tuning technique lies in the observation of the 100 most popular open-
source projects: more than 70\% are non-standalone functions, indicating that most functions in practice invoke or access non-built-in functions and non-standalone libraries.
From the view of code generation models, to generate non-standalone functions correctly, the docstring (natural language description) is not enough as the prompt for the model. Instead, contextual information is necessary and critical.
The model should be aware of the contextual information when inferencing, which requires it to be trained with such information as input.
However, since the previous models (i.e., Codex-S and PanGu-FT) are fine-tuned on only standalone functions to optimize the performance on HumanEval, they still lack the ability to make use of the context around the code to generate.
This gap motivates us to improve the existing pre-trained models through the fine-tuning stage.

We propose a \technique{} fine-tuning technique aims to resolve the following two questions:
We study two problems related to \technique{} fine-tuning: what to use as the context and how to combine it with the original prompt (i.e., the docstring).

For the first question, since the \wenwangdataset{} includes the enclosing file content for each function, we are able to use either the raw contextual code text (similar to what Copilot does) or the program analysis results as the contextual information~\cite{CHENG2022contextual1, kanade2020contextual2,wang2021contextual3}.
We experiment with both options and conclude that the first one was rather limited and unstable, especially for longer files and models with small window size (say 1024 for \codePLM).
Therefore, we adapt the second option and extract the contextual information in a simple but intuitive way, that is, parsing the file content into an AST and extracting the label of all import statements and definition nodes, and concatenating these labels according to the contextual information of the function. For example, for a function that contains tokens in the class, the imported library names and the class member signatures are concatenated as the context, as shown in Figure~\ref{fig.prompt}.
Additionally, we also divide the contextual information into two types: all\_context (all the contextual information in the current file) and oracle\_context (the actually-used contextual information in the ground truth solution), to study whether the model can learn to select the useful context correctly.

\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{figure/Prompt_Construction.pdf}
	\caption{An Example of Prompt with Context}
	\label{fig.prompt}
\end{figure}


For the second question, we experiment with 5 ways of combining the context with the original docstring to construct a new prompt for the model and adapt the best one to produce \wenwangcoder{}.
Specifically, the combinations include: \textit{all\_context + docstring}, \textit{docstring + all\_context}, \textit{docstring + all\_context + docstring}, \textit{oracle\_context + docstring}, \textit{docstring + oracle\_context}.
We use the \textit{only\_docstring} as the baseline for comparison, and process \wenwangdataset{} to 5 different versions, each of which replaces the original prompt with these new prompts.
Next, with the same hyper-parameters, we fine-tune \codePLM{} on these datasets independently to get 5 fine-tuned models and test their performance with the corresponding prompt format on \wenwangbench.
The result shows that: any combination of the contextual information and the docstring could improve the performance comparing \textit{only\_docstring}, while \textit{all\_context + docstring} brought the most significant improvements.
Surprisingly, we find that even prompting with other combinations, the model fine-tuned with \emph{all\_context+docs} still performs best and even better than the model specifically fine-tuned on that combination.
Therefore, we finally produce \wenwangcoder{} in this way.
Table~\ref{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts} shows the performance of different models fine-tuned on \codePLM{} by various context and docstring combinations.

Note that the performance of the model (short as WWDocs) fine-tuned with \textit{only\_docstring} is lower than that of PanGu-Coder, while the performance of other models (except \textit{docstring + all\_context} in Pass@1) is almost better than that of PanGu-Coder. This performance illustrates the importance of contextual information in generating code beyond standalone functions.
\begin{table}[th]
    \centering
    \footnotesize	
    \setlength\tabcolsep{1pt}
    \caption{Performance of models fine-tuned by various context and docstring combinations}
    \vspace*{-1.5ex}
    \label{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts}
    \begin{tabular}{@{}llrrr@{}} 
        \midrule
        Fine-tune Prompt Type & Inference Prompt Type & pass@1 & pass@5 & pass@10\\
        \midrule
        AllContext+Docs & AllContext+Docs & \textbf{14.43\%} & \textbf{22.29\%} & \textbf{25.65\%} \\
        \midrule
        Only Docs & Only Docs &  12.48\% & 19.06\% & 21.74\% \\
        \midrule
        Docs+AllContext & Docs+AllContext & 13.04\% & 21.31\% & 24.78\% \\
        \midrule
        Docs+AllContext+Docs & Docs+AllContext+Docs & 14.00\% & 20.65\% & 23.91\% \\
        \midrule
        OracleContext+Docs & OracleContext+Docs & 13.57\% & 20.86\% & 24.35\% \\
        \midrule
        Docs+OracleContext & Docs+OracleContext & 13.74\% & 20.26\% & 23.04\% \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 
% Due to the page limitation, we leave the detailed experiment results of models fine-tuned by various context and docstring combinations in the supplementary appendix.  
%值得注意的是，Only Docs模型的效果要低于PanGu-Coder，而其他模型的效果（除了Docs+AllContext的Pass@1）几乎都优于PanGu-Coder。这充分说明了在生成non-standalone函数时，提供上下文信息的重要性。

% Although we only fine-tuned \codePLM{} with our dataset and approach for experimentation, the idea can be applied to any pre-trained models to optimize their performance on the pragmatic generation of code.


==> dataavailability.tex <==
\section{Data Availability}
We have released all of the evaluation results on our anonymous website~\cite{sourcedata}.
We plan to publicly release our dataset at the publication time of our paper. 
At the current time of submission, we do not release our code repository as constrained by the public-disclosure requirement imposed  by our industrial collaborators at the moment; it would take some time to lift this requirement.


==> discussion.tex <==
\section{discussion}\label{sec:discussion}

We first discuss the performance of Codex\footnote{code-davinci-002.} on CoderEval and HumanEval.
Next, we discuss the possibility of applying our \technique{} fine-tuning technique on the pre-training stage.
Then, we discuss the limitation of Pass@K.
Finally, we show multiple examples for the code generated by the different models on CoderEval.

\begin{figure*}
    \subfigure[CodeGen and Pangu-Coder incorrect,  Wenwang-Coder correct]{
  \begin{minipage}[t]{0.3\linewidth}
   \centering
                \label{fig.case-one}
   \includegraphics[width=0.85\linewidth]{figure/appendix_case_1.pdf}
  \end{minipage}
 }
 \subfigure[CodeGen and Pangu-Coder incorrect, WWDocs and Wenwang-Coder correct]{
  \begin{minipage}[t]{0.3\linewidth}
   \centering
                \label{fig.case-two}
   \includegraphics[width=0.83\linewidth]{figure/appendix_case_2.pdf}
  \end{minipage}
 }
 \subfigure[CodeGen and Pangu-Coder correct,  Wenwang-Coder incorrect]{
  \begin{minipage}[t]{0.3\linewidth}
   \centering
                \label{fig.case-three}
   \includegraphics[width=1\linewidth]{figure/appendix_case_3.pdf}
  \end{minipage}
 }
\caption{Number of functions that models fail to solve with the original docstring but succeed with the human-labeled version}
\end{figure*}


\subsection{Comparison with Codex}
% \textbf{Compare with Codex\footnote{code-davinci-002.}}
We have also considered evaluating Codex but not compared Codex in Section~\ref{sec:experiments} for three reasons: (1) the original Codex paper did not open-source the model or the dataset, and (2) although the current Codex is accessible as a black box via OpenAI API, it only provides models of window size 2,048 and 8,000 according to the official documentation, which we estimate to be much larger than the 300M models in our experiments, and (3) although the GitHub Copilot plugin with Codex as the backend is publicly-available, we have no idea about the type and size of the online model.

For a more comprehensive comparison of experimental results, although comparing the 300M models used in this paper with Codex would be unfair, we still tried to use the latest version of Codex for comparison.
We use the code-davinci-002 of Codex for discussion. 
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1.4pt}
    \caption{Performance of different models (contains Codex) on 2 benchmarks}
    % Pass@K for \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} and HumanEval}
    \vspace*{-1.5ex}
    \label{tab: overall performance for wenwangbench and he with codex}
    \begin{tabular}{@{} ccc|ccccc @{}} 
        \toprule
        \multicolumn{1}{c}{\multirow{2.5}{*}{Benchmark}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Model}}
        & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
         \cmidrule(lr){3-6}
        & &  Pass@1(greedy) & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{\wenwangbench{}} & CodeGen &    10.87\%    & 9.26\% & 21.29\% & 25.22\% \\
        & \codePLM{} &  13.04\%  &   11.96\% & 19.73\% & 23.91\% \\
        & PanGu-FT &  13.48\%  &   13.09\% & 19.80\% & 22.61\% \\
        & \wenwangcoder{} & 16.09\%  & 14.43\% & 22.29\% & 25.65\% \\
        & Codex & 16.96\%  & 16.00\% & 26.72\% & 30.00\% \\
        \midrule
        \multirow{3}{*}{HumanEval} & CodeGen &   10.98\%     & 9.76\% & 18.85\% & 22.56\% \\
        & \codePLM{} &   17.07\%    & 13.23\% &20.46\% & 22.56\% \\
        &PanGu-FT &  15.85\%  &   14.57\% & 21.47\% & 23.78\% \\
        & \wenwangcoder{} &  17.68\% & 15.92\% & 21.76\% & 23.17\% \\
        & Codex  &  48.17\%  & 42.99\% & 72.04\% & 80.49\% \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 
Table~\ref{tab: overall performance for wenwangbench and he with codex} shows the performance of different models (contains Codex) on 2 benchmarks.
Both on HumanEval and \wenwangbench{}, Codex consistently outperforms the other four models.
The major reason is that Codex's model size is much larger than the other two models we tested. On HumanEval, Codex's numbers are much higher than other models and the original paper~\cite{codex}, indicating that HumanEval should not be used as a benchmark anymore due to overfitting or oversimplification.
% \textbf{Why \wenwangcoder{} fails on $slib\_depend$ and $plib\_depend$?}
% We find that correctly using the lib is the most difficult thing in context-aware code generation, due to the following 4 steps: choosing the correct library, choosing the correct API, generating the correct invocation arguments, and using the return value or effect correctly. We are trying the most difficult scenario (i.e., given all possible libraries in the current file), so the results are reasonable. However, our approach does bring improvements on both class-level and file-level, since correctly choosing and utilizing variables and functions in the current class and current file is essentially easier, since the search space is much smaller.

% \subsection{Applying the \technique{} fine-tuning technique in the pre-training stage}
% In this paper, we do experiments with the \technique{} fine-tuning technique in the fine-tuning stage.
% Since we can use the same way to extract the all\_context information and oracle\_context information in the pre-training data,
% the \technique{} fine-tuning technique may also be useful in the pre-training stage.
% We will do this experiment in our future work.

\subsection{Pre-training with our \technique{} fine-tuning technique}
% \textbf{Pre-training with sliced context.}
Inspired by the improved performance of \wenwangcoder{} after adding the extracted contextual information, we believe that the idea can also be applied in the pre-training stage.
Existing generative language models of code (like Codex and CodeGen) still follow the self-supervised pre-training way of natural language, they treat source code as plain text but ignore the structure of code elements.
Considering that the order of source code does not necessarily indicate the causal relationship, we conjecture that the plain casual language modelling is not the best approach to pre-training the language model of code, it is worth trying to apply software analysis techniques in the pre-training stage, for example, slicing relevant context according to heuristic rules.
We think the \technique{} fine-tuning technique may also be useful in the pre-training stage.
We will do this experiment in our future work.


\subsection{Limitation of Pass@K}
%\textbf{Limitation of Pass@K.} 
Although Pass@K is widely adopted, it still has several limitations.
During our research, we note two major limitations: (1) it heavily relies on the quality of test cases. Test cases with low coverage or missing corner cases can lead to false positives (programs that pass all tests but are not actually correct)~\cite{alpha_code}, and (2) it requires the function to have explicit input (arguments) and output (return values), but there are many functions without input or output in real projects.
To stay close to the fact, \wenwangbench{} includes 38 functions without input or output values, for which we try to evaluate the behavioral correctness by checking the expected effect as the test cases. However, it is still difficult to strictly determine the correctness of such functions, which we leave as the future optimization for the benchmark. We additionally evaluate the three models only on those functions with explicit return values and find the result leads to the same conclusion as Section~\ref{sec.rq1}.







\subsection{Case study.}



Figure ~\ref{fig.case-one} shows the code generated by different models with all context and docstring as inputs. The code generated by CodeGen and Pangu-Coder fails to pass the test cases in the WenwangBench, but the code generated by Wenwang-Coder can pass the test cases.
% \begin{figure}[th]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{figure/appendix_case_1.pdf}
% 	\caption{Case Study \uppercase\expandafter{\romannumeral1}}
% 	\label{fig.case-one}
% \end{figure}

Figure ~\ref{fig.case-two} shows the code generated by four different models with only docstring as input, where CodeGen and Pangu-Coder failed the test cases of CoderEval. Significantly, the WWDocs can pass the test cases of WenwangBench even if only docstring is available.

% \begin{figure}[th]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{figure/appendix_case_2.pdf}
% 	\caption{Case Study \uppercase\expandafter{\romannumeral2}}
% 	\label{fig.case-two}
% \end{figure}

Figure ~\ref{fig.case-three} shows the case where Wenwang-Coder failed the test cases with only docstring as input, and the other two models passed. However, as we can see, the code generated by WenwangCoder is similar to oracle code with only a few errors and still conforms to what docstring expresses.


% \begin{figure}[th]
% 	\centering
% 	\includegraphics[width=0.8\linewidth]{figure/appendix_case_3.pdf}
% 	\caption{Case Study \uppercase\expandafter{\romannumeral3}}
% 	\label{fig.case-three}
% \end{figure}

% \textbf{Why}
% \subsection{Generating functions with Non-null return value}

% In Section~\ref{sec:experiment results}, we discussed and analyzed the overall and six runnable levels performance of three models on \wenwangbench{}. 
% Here we discuss the proportion of functions with none return value in \wenwangbench{} and the experimental results after removing these functions in \wenwangbench{}.
% In totally, 38 functions in \wenwangbench{} has none return type.
% In realistic development scenarios, many functions do not have return values. 
% Since \wenwangbench{} is built from open-source projects, some functions do not have return values. 
% For these functions with none return value, we do not think it is correct to force a return value to them, because the model can also generate many functions with none return value. So we keep these functions in \wenwangbench{}, and in the previous experiments, we considered them correct as long as the code generated by models for these functions with none return value had a return value of none and had no error in the code execution. 
% % This ensures that we may miss the wrong program, but not the right one.
% In this section, we remove the functions whose return value is None from the \wenwangbench{} and then test the effects of the three models on it. 
% Experiment results show that the overall performance of \wenwangcoder{} is also higher than that of CodeGen and \codePLM{} after removing the functions whose return value is None.
% \wenwangcoder{} outperforms CodeGen by 4.74\% when generating only one solution, and by 2.09\% when recommending one from 10 generated solutions.
% Comparing with \codePLM{}, \wenwangcoder{} brings an improvement of 1.51\% when generating only one solution, and 1.04\% when generating 10 solutions.
% % Compared with Table~\ref{tab: overall performance for wenwangbench and he}, after excluding the functions with none return type in \wenwangbench{}, all models have a slight decrease in effectiveness.
% we leave detail results on 6 runnable levels of \wenwangbench{} 


==> evaluation/rq1.tex <==

    %Overall performance
    %venn complenmentary and union
    %ablation study for wenwang-coder with wenwang-only-docs
    %ablation study for pangu-ft with wenwang-only-docs
    %Compare the effectiveness of different models in correctly utilizing the contextual information on \wenwangbench{}
\subsection{RQ1: How does \wenwangcoder{} compare against publicly available code generation models on \wenwangbench{} and HumanEval?}
We first show the overall performance of \wenwangcoder{} against other models on HumanEval and \wenwangbench{}.
Next, we show the complementarity of the number of correct generating functions between the different models.
Then, we conduct an ablation experiment for \wenwangcoder{}, WWDocs, and PanGu-FT, to analyze the effectiveness of our \technique{} technique.
Next, we detail the performance of different models between standalone and non-standalone functions in \wenwangbench{}.
Finally, we show the performance of different models in correctly utilizing the contextual information on \wenwangbench{}.

\subsubsection{Overall performance}
\label{sec.rq1}

Table~\ref{tab: overall performance for wenwangbench and he} shows the overall performance of \wenwangcoder{} against other models on HumanEval and \wenwangbench{}.
Besides the performance of PanGu-FT on HumanEval (Pass@10), \wenwangcoder{} consistently outperforms CodeGen, \codePLM{}, and PanGu-FT at all Pass@Ks on both \wenwangbench{} and HumanEval.~\footnote{HumanEval scores are slightly different from the CodeGen and \codePLM{} paper because they used \emph{n}=200 in experiments.}
On \wenwangbench{}, \wenwangcoder{} outperforms CodeGen by 5.22\% when generating only one solution and by 5.17\% when recommending one from 10 generated solutions.
Comparing with its baseline model \codePLM{}, \wenwangcoder{} brings an improvement of 3.05\% on Pass@1 (greedy), and 2.47\%, 2.56\%, 1.74\% when generating 10 solutions.
Although \wenwangcoder{} is designed to enhance the capability to generate non-standalone functions, the standalone function generation ability inherited from \codePLM{} does not degrade on HumanEval.
Comapring with another fine-tuned model on \codePLM{} model PanGu-FT, \wenwangcoder{}, \wenwangcoder{} brings an improvement of 3.05\% on Pass@1 (greedy), and 1.34\%, 2.49\%, 3.04\% when generating 10 solutions.
Since PanGu-FT is fine-tuned with only standalone functions, PanGu-FT outperforms other models on HumanEval.  
In a conclusion, experimental results show that \wenwangcoder{} not only outperforms the fine-tuned model (i.e., PanGu-FT) but also outperforms the pre-trained models (i.e., CodeGen and \codePLM{}), demonstrate the benefits and performance of \wenwangcoder{}.

% From the table, we can also observe that on \wenwangbench{}, CodeGen is less effective than \codePLM{} at Pass@1, but outperforms \codePLM{} at Pass@5 and Pass@10. 
% In addition, the gap between CodeGen at Pass@5 and Pass@10 metrics is narrowed compared to Wenwang at Pass@1 performance.
% This shows that CodeGen is more capable of generating diverse code than \codePLM{}.

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1.4pt}
    \caption{Main Results for 4 Models on 2 Benchmarks}
    % Pass@K for \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} and HumanEval}
    \vspace*{-1.5ex}
    \label{tab: overall performance for wenwangbench and he}
    \begin{tabular}{@{} ccc|ccccc @{}} 
        \toprule
        \multicolumn{1}{c}{\multirow{2.5}{*}{Benchmark}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Model}}
        & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
         \cmidrule(lr){3-6}
        & &  Pass@1(greedy) & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{\wenwangbench{}} & CodeGen &    10.87\%    & 9.26\% & 21.29\% & 25.22\% \\
        & \codePLM{} &  13.04\%  &   11.96\% & 19.73\% & 23.91\% \\
        & PanGu-FT &  13.48\%  &   13.09\% & 19.80\% & 22.61\% \\
        & \wenwangcoder{} & \textbf{16.09\%}  & \textbf{14.43\%} & \textbf{22.29\%} & \textbf{25.65\%} \\
        \midrule
        \multirow{3}{*}{HumanEval} & CodeGen &   10.98\%     & 9.76\% & 18.85\% & 22.56\% \\
        & \codePLM{} &   17.07\%    & 13.23\% &20.46\% & 22.56\% \\
        & PanGu-FT &  15.85\%  &   14.57\% & 21.47\% & 23.78\% \\
        & \wenwangcoder{} &  \textbf{17.68\%}  & \textbf{15.92\%} & \textbf{21.76\%} & \textbf{23.17\%} \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 



\subsubsection{Complementarity between the different models}\label{sec:comall}

Figure~\ref{fig.complenment_overall} shows the number of solved problems by the different models on \wenwangbench{}, with the difference and overlapping.
We consider a problem to be solved if the model can generate \emph{at least} one correct solution that passes all tests out of the ten generated solutions.
Figure~\ref{fig.complenment_overall_pretrain} shows the difference and overlapping between \wenwangcoder{} with pre-trained models (i.e., CodeGen and \codePLM{}). 
Among the 230 problems in \wenwangbench{}, the total number of problems solved by the three models is 72 (union), while 41 (intersection) problems can be solved by any of the three models.
Figure~\ref{fig.complenment_overall_finetune} shows the difference and overlapping between \wenwangcoder{} with fine-tuned models.
Among the 230 problems in \wenwangbench{}, the total number of problems solved by the three models is 68 (union), while 37 (intersection) problems can be solved by any of the three models.
% Among the 68 questions that the three models can solve correctly, \wenwangcoder{} can solve 59 questions correctly, while the other two models can only generate 50 and 52 questions correctly.
% Experimental result shows the effectiveness of \wenwangcoder{}.
The high intersection (e.g., 41 and 37 problems in Figure~\ref{fig.complenment_overall_pretrain} and ~\ref{fig.complenment_overall_finetune}, respectively) of correctly generated code by different models shows that different models can generate code correctly for some problems, indicating that the basic generation ability of each model is good.
The high complementarity (e.g., 72 and 68 problems in Figure~\ref{fig.complenment_overall_pretrain} and ~\ref{fig.complenment_overall_finetune}, respectively) of all models shows how combining different models deserve more research attention.

\begin{figure}
\centering
\subfigure[\wenwangcoder{} with pre-trained models]{
\label{fig.complenment_overall_pretrain}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{figure/mainpretraincom.pdf}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[\wenwangcoder{} with fine-tuned models ]{
\label{fig.complenment_overall_finetune}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{figure/mainfinetunecom.pdf}
\end{minipage}%
}%
\centering
\caption{Number of correctly-generated functions of different models on \wenwangbench{}}
\label{fig.complenment_overall}
\end{figure}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.5\linewidth]{figure/complementarity-overall.pdf}
% 	\caption{Number of correctly-generated functions of CodeGen, \codePLM{}, and \wenwangcoder{} on \wenwangbench{}}
% 	\label{fig.complenment_overall}
%  \vspace*{-2.5ex}
% \end{figure}

\subsubsection{Ablation study for \wenwangcoder{}, WWDocs, and PanGu-FT}
To analyze the impact of \wenwangdataset{} for fine-tuned model and the effectiveness of our \technique{} technique, we conduct an ablation experiment for \wenwangcoder{}, WWDocs, and PanGu-FT.
The WWDocs model corresponds to the model in the second line in Table~\ref{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts}.
WWDocs model uses the traditional fine-tuning technique (i.e., the input for fine-tuning WWDocs is only docstring), it does not use any contextual information of the function in the fine-tuning dataset.
% We compare the performance of \wenwangcoder{} and WWDocs to show the effectiveness of the \technique{} fine-tuning technique.

Both \wenwangcoder{} and WWDocs are all fine-tuned on \codePLM{} based on \wenwangdataset{}, the difference between \wenwangcoder{} and WWDocs is that \wenwangcoder{} additionally applies the \technique{} technique proposed in this paper and additionally uses the contextual information for fine-tuning.
Table~\ref{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts} and ~\ref{tab: overall performance for wenwangbench and he} show that \wenwangcoder{} outperforms WWDocs on \wenwangbench{}, which demonstrates the effectiveness of the proposed \technique{} technique.

Compared with Pangu-FT, WWDocs also perform better in all Pass@K.
Both WWDocs and PanGu-FT are all fine-tuned on \codePLM{} with the original docstring (without the contextual information and the \technique{} technique proposed in this paper), the difference between WWDocs and PanGu-FT is that WWDocs is not only used the standalone functions for fine-tuning but also used the non-standalone functions.
Interestingly, the performance of PanGu-FT and WWDocs is fairly close, which shows that only docstring is not enough when generating non-standalone functions. An effective way is to use the contextual information of the function in both the pre-training and inferencing stages.
%PanGu-FT和WWDocs的效果很接近，这说明了生成non-standalone function时只用docstring是不够的，在训练和推理阶段最好都使用程序的上下文信息。
%Table~\ref{tab: The performance of wenwangcoder finetuned on different prompt and on different input prompts} and ~\ref{tab: overall performance for wenwangbench and he} show that the performance of Wenwang-onlydocs and PanGu-FT is similar.
%Analyze reasons.xxx


\subsubsection{The performance of different models between standalone functions with non-standalone functions in \wenwangbench{}}
% Table~\ref{tab: mult performance on wenwangbench} shows the performance of three models on the six types of functions in \wenwangbench{}.
% % The type of function represents the non-overlapping part between two neighboring runnable levels in Figure~\ref{fig.run_dep_res}. For example, the class\_depended represents those functions that must depend on other code in the current class.
% While \wenwangcoder{} outperforms CodeGen and \codePLM{} at self\_contained, class\_depended, and file\_depended levels, it slightly downgrades at slib\_depended, plib\_depended, and project\_depended levels, which is consistent with the above case study on the 4 cases that \codePLM{} succeeds but \wenwangcoder{} fails.
% By comparing the generated code manually, we find that \wenwangcoder{} is more capable of understanding and using the provided context to generate code compared with the other models.
% Particularly, at the class\_depended and file\_depended level, where the function is expected to use the existing code in the current class or file, \wenwangcoder{} is better at selecting and using the correct functions and variables, so it obviously outperforms \codePLM{} by a large margin.
% However, at the slib\_depended and plib\_depended level where the function is expected to use the API provided by libraries, \wenwangcoder{} seems to be overwhelmed by the contextual information that tells it all the imported library names.
% As there are many libraries and APIs in each library to choose from, it is difficult for the model to make the correct choice, although it seems simple and straightforward for experienced developers.
% Based on this observation, we anticipate that it is a promising research direction to integrate API recommendation tools~\cite{Rahman2016APIreco1, huang2018APIreco2, li2018APIreco3} to recommend a set of possibly-used libraries/APIs as the context, which will significantly reduce the decoding space of large language models when in generating code beyond standalone functions.


% \begin{table}[t]
%     \centering
%     \footnotesize	
%     \caption{Performance of 3 Models Across 6 Types of functions}
%     \vspace*{-1.5ex}
%     \label{tab: mult performance on wenwangbench}
%     \begin{tabular}{@{}rcrrrrrrrr@{}} 
%         \midrule
%         Runnable Level &  \multicolumn{1}{c}{Model}  & Pass@1 & Pass@5 & Pass@10\\
%         \midrule
%         \multirow{3}{*}{self\_contained} &  CodeGen  &  17.14\% & 34.82\% & 37.14\% \\
%         & \codePLM{} & 21.14\% &34.92\% & 40.00\% \\
%         & PanGu-FT & 18.86\% &32.06\% & 37.14\% \\
%         & \wenwangcoder{} & \textbf{28.00\%} & \textbf{39.85\%} & \textbf{42.86\%} \\
%         \midrule
%         \multirow{3}{*}{slib\_depended} &  CodeGen  & 8.21\% & 20.04\% & 25.00\% \\
%         & \codePLM{} &  \textbf{12.50\%} & \textbf{24.89\%} & \textbf{32.14\%} \\
%         & PanGu-FT & 12.86\% &26.02\% & 32.14\% \\
%         & \wenwangcoder{} & 12.14\% & 20.55\% & 25.00\% \\
%         \midrule
%         \multirow{3}{*}{plib\_depended} & CodeGen & 9.52\% & 25.57\% & \textbf{33.33\%} \\
%         & \codePLM{} & \textbf{16.67\%} & \textbf{27.49\%} & \textbf{33.33\%} \\
%         & PanGu-FT & 13.33\% &18.65\% & 19.05\% \\
%         & \wenwangcoder{} & 14.76\% & 21.32\% & 23.81\% \\
%         \midrule
%         \multirow{3}{*}{class\_depended} & CodeGen & 9.82\% & 24.24\% & 29.09\% \\
%         & \codePLM{} & 10.55\% & 17.98\% & 23.64\% \\
%         & PanGu-FT & 13.45\% &19.36\% & 21.82\% \\
%         & \wenwangcoder{} & \textbf{17.45\%} & \textbf{27.02\%} & \textbf{30.91\%} \\
%         \midrule
%         \multirow{3}{*}{file\_depended} & CodeGen &  7.50\% & \textbf{16.15\%} & \textbf{19.12\%} \\
%                 & \codePLM{} & 9.85\% & 12.91\% & 14.71\% \\
%                 & PanGu-FT & 13.24\% &16.88\% & 19.12\% \\
%         & \wenwangcoder{} & \textbf{10.15\%} & 15.90\% & \textbf{19.12\%} \\
%         \midrule
%         \multirow{3}{*}{project\_depended} & CodeGen & 2.17\% & 6.42\% & \textbf{8.70\%} \\
%         & \codePLM{} & \textbf{2.61\%} & \textbf{7.63\%} & \textbf{8.70\%} \\
%         & PanGu-FT & 3.04\% &4.35\% & 4.35\% \\
%         & \wenwangcoder{} & 1.74\% & 6.16\% &  \textbf{8.70\%} \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-2.5ex}
% \end{table}

\begin{table}[t]
% \vskip 0.3in
    \centering
    \footnotesize	
    \caption{Performance of different models between standalone functions and non-standalone functions in \wenwangbench{}}
   
    \vspace*{-1.5ex}
    \label{tab: ss and others performance on wenwangbench}
    \begin{tabular}{@{}rcrrrrr@{}} 
        \midrule
         Dependency &   Model & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{standalone} &  CodeGen  &  13.17\% & 28.25\% & 31.74\% \\
        & \codePLM{} &17.30\% &30.46\% & 36.51\% \\
        & PanGu-FT &16.19\% &29.38\% & 34.92\% \\
        & \wenwangcoder{} &20.95\% & 34.27\% & 34.92\% \\
        \midrule
        \multirow{3}{*}{non-standalone} &  CodeGen  & 7.78\% & 18.66\% & 22.76\% \\
        & \codePLM{} &  9.94\% & 15.69\% & 19.16\% \\
        & PanGu-FT &11.92\% &16.19\% & 17.80\% \\
        & \wenwangcoder{} &11.98\% & 18.90\% & 22.16\% \\

        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table}
To explore the performance of \wenwangcoder{} in generating the non-standalone functions, we further compare the performance of \wenwangcoder{} with other models in generating the standalone functions (slib\_runnable subset of \wenwangbench{}) and non-standalone functions (other runnable-levels).
%Table~\ref{tab: ss and others performance on wenwangbench} shows the performance of different models between standalone functions and non-standalone functions in \wenwangbench{}.
As shown in Table~\ref{tab: ss and others performance on wenwangbench}, \wenwangcoder{} outperforms other models on both standalone and non-standalone functions, demonstrating the effectiveness of \wenwangcoder{}.

In addition, the performance of all models in generating the standalone functions is substantially higher than that of non-standalone functions.
Considering that more than 70\% of real functions are non-standalone functions, improving the model's ability to consider and use contextual information correctly is vital for the practical value of such technology.

% It is worth noting that all models perform very poorly at the project\_runnable level, which is not surprising considering the commonly-adopted self-supervised and auto-regressive pre-training method.
% Currently, almost all these large generative models of code follow the architecture and training approach in natural language processing. They consider the source code as plain text and pre-trained a causal language model with the next-token prediction within a source file. However, considering the cross-file context information in the prompt is necessary for generating code beyond standalone functions in real projects, as a recent exploration study~\cite{repo_level} shows. We consider it to be our future work on a more \emph{intelligent} \techique{} code generation.

\subsubsection{The performance of different models correctly utilises the contextual information.}

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2pt}
    \caption{Accuracy of different models that they can correctly generate the contextual tokens}
    \vskip 0.15in
    \label{tab: contextual}
    \begin{tabular}{@{} cc|cccccccc @{}} % suppress vertical whitespace at start and end
        \toprule
        % \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Prompt}} 
        % & & \multicolumn{4}{c}{Python} & \multicolumn{4}{c}{Java} &
        \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Contextual Type}}  & \multicolumn{3}{c}{Acc@K}\\
        \cmidrule(lr){3-5} 
        % & & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}& \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
        %  \cmidrule(lr){4-6}  \cmidrule(lr){8-10}
         & & Acc@1 & Acc@5 & Acc@10\\
        \midrule
        \multirow{3}{*}{CodeGen} &  TypeReference  &  12.63\% &  22.97\% & 25.93\% \\
        & APIInvocation   &  7.78\%& 17.40\% & 21.90\%\\
        & VarReference   & 3.37\%  & 7.10\% &8.36\%\\
        \midrule
        \multirow{3}{*}{\codePLM} &  TypeReference  & 13.16\%&  22.80\% & 26.46\% \\
        & APIInvocation   & 6.64\%& 11.22\% & 14.53\% \\
        & VarReference  &3.15\%& 4.60\% & 5.30\% \\
        \midrule
        \multirow{3}{*}{PanGu-FT} &  TypeReference  & 12.67\%&  21.06\% & 22.60\% \\
        & APIInvocation   & 7.72\%& 13.03\% & 14.81\% \\
        & VarReference  &2.95\%& 3.20\% & 3.45\% \\
        \midrule
        \multirow{3}{*}{\wenwangcoder{}} &  TypeReference   & 15.81\%&  23.58\% & 29.73\% \\
        & APIInvocation   & 10.57\%&17.51\% &20.83\%\\
        & VarReference   & 6.83\%& 10.83\% & 12.62\%\\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
    
\end{table} 

% To further compare the \emph{context-awareness} of \wenwangcoder{} to other state-of-the-art models, we analyze the identifier tokens in generated code and focus on three types of tokens: TypeReference, APIInvocation, and VarReference (including constants reference).
% Table~\ref{tab: contextual} shows the Acc@k of all models, we find it is consistent with Pass@K (i.e., the generated functions can pass test cases), and the Acc@K of \wenwangcoder{} is also the best one in generating contextual dependency. 
%一个重要的原因是\wenwangcoder{}在推理和训练阶段都显示的接受了上下文信息作为输入。
To further explore the ability of different models in generating different types of contextual information, similar to the experiments in CoderEval~\cite{yu2023ce}, we divide the context token into three categories: TypeReference, APIInvocation, and VarReference, which usually form the most important part of the implementation at runnable-levels (defined in CoderEval) with external dependency.
%We do not classify constants because, in common programming habits, developers often use a global variable declaration for a constant, which is context-dependent. 
Table~\ref{tab: contextual} shows the Acc@k of all models, we find it is consistent with Pass@K (i.e., the generated functions can pass test cases), and the Acc@K of \wenwangcoder{} is also the best one in generating contextual dependency. 
After analyzing the reasons, we think that \wenwangcoder{} has accepted the contextual information as input in the inferencing and fine-tuning stages.
Thus, how to combine the correctly generated context information more effectively is a worthy research direction.

In addition, as shown in Table~\ref{tab: contextual}, on \wenwangbench{}, all models show poor effectiveness in generating the correct ``VarReference'' token, while the effectiveness in generating the ``TypeReference'' token is relatively good.
When generating Python functions, studying how to better generate ``VarReference'' tokens may be an effect way to improve the code generation ability of the model.

==> evaluation/rq1_back.tex <==
% \subsection{RQ1: How do CodeGen, \codePLM{}, and \wenwangcoder{} perform on HumanEval and \wenwangbench{}?}
\subsection{RQ1: How do \wenwangcoder{}, PanGu-FT, and other two pre-trained models perform on HumanEval and \wenwangbench{}?}
% In this section, we first show the overall performance of \codePLM{}, CodeGen, and \wenwangcoder{} on HumanEval and \wenwangbench{}.
% Then we show the complementarity of the number of correct generating functions between the 3 models.
% Finally, we detail the different performance of the 3 models with multi-variants combination of contextual information.

\subsubsection{Overall performance}
\label{sec.rq1}

Table~\ref{tab: overall performance for wenwangbench and he} shows the overall performance of CodeGen, \codePLM{}, and \wenwangcoder{} on HumanEval and \wenwangbench{}. 
\wenwangcoder{} consistently outperforms CodeGen and \codePLM{} at all Pass@Ks on both \wenwangbench{} and HumanEval.~\footnote{HumanEval scores are slightly different from the CodeGen and \codePLM{} paper because they used \emph{n}=200 in experiments.}
On \wenwangbench{}, \wenwangcoder{} outperforms CodeGen by 5.22\% when generating only one solution and by 5.17\% when recommending one from 10 generated solutions.
Comparing with its baseline model \codePLM{}, \wenwangcoder{} brings an improvement of 3.05\% on Pass@1 (greedy), and 2.47\%, 2.56\%, 1.74\% when generating 10 solutions.
Although \wenwangcoder{} is designed to enhance the capability to generate non-standalone functions, the standalone function generation ability inherited from \codePLM{} does not degrade on HumanEval.

% From the table, we can also observe that on \wenwangbench{}, CodeGen is less effective than \codePLM{} at Pass@1, but outperforms \codePLM{} at Pass@5 and Pass@10. 
% In addition, the gap between CodeGen at Pass@5 and Pass@10 metrics is narrowed compared to Wenwang at Pass@1 performance.
% This shows that CodeGen is more capable of generating diverse code than \codePLM{}.

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1.4pt}
    \caption{RQ1: Main Results for 3 Models on 2 Benchmarks}
    % Pass@K for \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} and HumanEval}
    \vspace*{-1.5ex}
    \label{tab: overall performance for wenwangbench and he}
    \begin{tabular}{@{} ccc|ccccc @{}} 
        \toprule
        \multicolumn{1}{c}{\multirow{2.5}{*}{Benchmark}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Model}}
        & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
         \cmidrule(lr){3-6}
        & &  Pass@1(greedy) & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{\wenwangbench{}} & CodeGen &    10.87\%    & 9.26\% & 21.29\% & 25.22\% \\
        & \codePLM{} &  13.04\%  &   11.96\% & 19.73\% & 23.91\% \\
        & PanGu-FT &  -\%  &   13.09\% & 19.80\% & 22.61\% \\
        & \wenwangcoder{} & \textbf{16.09\%}  & \textbf{14.43\%} & \textbf{22.29\%} & \textbf{25.65\%} \\
        \midrule
        \multirow{3}{*}{HumanEval} & CodeGen &   10.98\%     & 9.76\% & 18.85\% & 22.56\% \\
        & \codePLM{} &   17.07\%    & 13.23\% &20.46\% & 22.56\% \\
        & PanGu-FT &  -\%  &   19.50\% & -\% & 25.96\% \\
        & \wenwangcoder{} &  \textbf{17.68\%}  & \textbf{15.92\%} & \textbf{21.76\%} & \textbf{23.17\%} \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 


\subsubsection{Detailed Comparison}

Figure~\ref{fig.complenment_overall} shows the number of solved problems by the three models on \wenwangbench{}, with the difference and overlapping.
We consider a problem to be solved if the model can generate \emph{at least} one correct solution that passes all tests out of the ten generated solutions.
Among the 230 problems in \wenwangbench{}, the total number of problems solved by the three models is 88 (union), while 48 problems can be solved by any of the three models (intersection).
Compared with \codePLM{}, \wenwangcoder{} additionally solves 11 different problems, while failing to solve four that \codePLM{} should have solved. We dive into the concrete cases and find that three of them rely on standard or public libraries (one slib\_runnable and two plib\_runnable). For these problems, although \wenwangcoder{} is prompted with the imported libraries in the current file, it fails to use the correct library or API to fulfill the correct implementation.


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figure/complementarity-overall.pdf}
	\caption{Number of correctly-generated functions of CodeGen, \codePLM{}, and \wenwangcoder{} on \wenwangbench{}}
	\label{fig.complenment_overall}
 \vspace*{-2.5ex}
\end{figure}

 


Table~\ref{tab: mult performance on wenwangbench} shows the performance of three models on the six types of functions in \wenwangbench{}.
The type of function represents the non-overlapping part between two neighboring runnable levels in Figure~\ref{fig.run_dep_res}. For example, the class\_depended represents those functions that must depend on other code in the current class.
While \wenwangcoder{} outperforms CodeGen and \codePLM{} at self\_contained, class\_depended, and file\_depended levels, it slightly downgrades at slib\_depended, plib\_depended, and project\_depended levels, which is consistent with the above case study on the 4 cases that \codePLM{} succeeds but \wenwangcoder{} fails.
By comparing the generated code manually, we find that \wenwangcoder{} is more capable of understanding and using the provided context to generate code compared with the other models.
Particularly, at the class\_depended and file\_depended level, where the function is expected to use the existing code in the current class or file, \wenwangcoder{} is better at selecting and using the correct functions and variables, so it obviously outperforms \codePLM{} by a large margin.
However, at the slib\_depended and plib\_depended level where the function is expected to use the API provided by libraries, \wenwangcoder{} seems to be overwhelmed by the contextual information that tells it all the imported library names.
As there are many libraries and APIs in each library to choose from, it is difficult for the model to make the correct choice, although it seems simple and straightforward for experienced developers.
Based on this observation, we anticipate that it is a promising research direction to integrate API recommendation tools~\cite{Rahman2016APIreco1, huang2018APIreco2, li2018APIreco3} to recommend a set of possibly-used libraries/APIs as the context, which will significantly reduce the decoding space of large language models when in pragmatic code generation.


\begin{table}[t]
    \centering
    \footnotesize	
    \caption{Performance of 3 Models Across 6 Types of functions}
    \vspace*{-1.5ex}
    \label{tab: mult performance on wenwangbench}
    \begin{tabular}{@{}rcrrrrrrrr@{}} 
        \midrule
        Runnable Level &  \multicolumn{1}{c}{Model}  & Pass@1 & Pass@5 & Pass@10\\
        \midrule
        \multirow{3}{*}{self\_contained} &  CodeGen  &  17.14\% & 34.82\% & 37.14\% \\
        & \codePLM{} & 21.14\% &34.92\% & 40.00\% \\
        & \wenwangcoder{} & \textbf{28.00\%} & \textbf{39.85\%} & \textbf{42.86\%} \\
        \midrule
        \multirow{3}{*}{slib\_depended} &  CodeGen  & 8.21\% & 20.04\% & 25.00\% \\
        & \codePLM{} &  \textbf{12.50\%} & \textbf{24.89\%} & \textbf{32.14\%} \\
        & \wenwangcoder{} & 12.14\% & 20.55\% & 25.00\% \\
        \midrule
        \multirow{3}{*}{plib\_depended} & CodeGen & 9.52\% & 25.57\% & \textbf{33.33\%} \\
        & \codePLM{} & \textbf{16.67\%} & \textbf{27.49\%} & \textbf{33.33\%} \\
        & \wenwangcoder{} & 14.76\% & 21.32\% & 23.81\% \\
        \midrule
        \multirow{3}{*}{class\_depended} & CodeGen & 9.82\% & 24.24\% & 29.09\% \\
        & \codePLM{} & 10.55\% & 17.98\% & 23.64\% \\
        & \wenwangcoder{} & \textbf{17.45\%} & \textbf{27.02\%} & \textbf{30.91\%} \\
        \midrule
        \multirow{3}{*}{file\_depended} & CodeGen &  7.50\% & \textbf{16.15\%} & \textbf{19.12\%} \\
                & \codePLM{} & 9.85\% & 12.91\% & 14.71\% \\
        & \wenwangcoder{} & \textbf{10.15\%} & 15.90\% & \textbf{19.12\%} \\
        \midrule
        \multirow{3}{*}{project\_depended} & CodeGen & 2.17\% & 6.42\% & \textbf{8.70\%} \\
        & \codePLM{} & \textbf{2.61\%} & \textbf{7.63\%} & \textbf{8.70\%} \\
        & \wenwangcoder{} & 1.74\% & 6.16\% &  \textbf{8.70\%} \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table}

It is worth noting that all models perform very poorly at the project\_runnable level, which is not surprising considering the commonly-adopted self-supervised and auto-regressive pre-training method.
Currently, almost all these large generative models of code follow the architecture and training approach in natural language processing. They consider the source code as plain text and pre-trained a causal language model with the next-token-prediction within a source file. However, considering the cross-file context information in the prompt is necessary for pragmatic code generation in real projects, as a recent exploration study~\cite{repo_level} shows. We consider it to be our future work on a more \emph{intelligent} context-aware code generation.

% After the functions and variables related to the class and the current file are added in the finetune phase and code generation phase, \wenwangcoder{} can select the correct functions and variables in the current class and file to invoke, thereby improving the accuracy of code generation in the class\_runnable, and file\_runnable levels.

% After analyzing reasons, we think that it is not enough to introduce only the context information of the standard library and the public library, because each library may call many functions and variables, so it is difficult for the large language models to make a correct choice. 
% It would be an interesting research direction to recommend the functions and variables that may be called in the library based on the program context information and natural language description.

% Note that \codePLM{} outperforms CodeGen and \wenwangcoder{} on project\_level.
% This is not common sense, because for all models, finetune is only done at the file level, and pangu does not make sense to be more effective at the project\_runnable level than the CodeGen and \wenwangcoder{}. 
% According to the example analysis, all models generate incorrect answers at the project\_runnable level. 
% The reason why our verification platform judge these answers as correct is the return value of the test cases corresponding to these answers is None. 
% Therefore, the generated code is considered correct as long as no error is reported and no return value is returned during running.

% In Section~\ref{sec:discussion}, we will describe in detail the ratio of functions that do not return values to \wenwangbench{} and the experimental results after these functions are removed. 
% We find that the proportion of these functions is small, and our conclusions remain unchanged after removing these functions.

==> evaluation/rq2.tex <==
\subsection{RQ2: How does the performance of different models vary on different context types and formats on \wenwangbench{}?}

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figure/experient_ablation_big.pdf}
	\caption{The performance of CodeGen, \codePLM{}, PanGu-FT, and \wenwangcoder{} on \wenwangbench{} with 5 combinations of the contextual information and docstring in inferencing stage}
	\label{fig: experimentAblation}
\end{figure*}
% Figure~\ref{fig: experimentAblation} shows examples of different information combinations and the effects of \codePLM{}, CodeGen, and \wenwangcoder{} on them.
We conduct an ablation experiment to study the effect of different types and formats of context for different models.
Figures~\ref{fig: experimentAblation} shows the performance of CodeGen, \codePLM{}, PanGu-FT, and \wenwangcoder{} on 5 combinations of the contextual information and the docstring (see Section~\ref{sec: wenwang} for details).
The first row in this figure shows the performance when adding all the available context (all\_context) in the prompt, and the second row shows the results when adding only the actually-used context in the ground truth code (oracle\_context).
In the practical scenario, the all\_context can be analyzed through program analysis, but the oracle\_context is actually unavailable since there is no oracle solution, so we just use the experiment to study the ability of models to \emph{consume} the correct contextual information.

% Since it is difficult to obtain oracle information automatically in realistic development, we list the two combinations involving oracles separately (The upper part of Figure~\ref{fig: experimentAblation} shows the result that does not contain the Oracle information. The lower part of Figure~\ref{fig: experimentAblation} shows the result that contains the oracle information).

Among the 4 models, \wenwangcoder{} consistently exhibits better performance, regardless of the way to combine the context and the docstring.
Among the 5 combinations, the all\_context + docstring combination is the best at all of Pass@1, Pass@5, and Pass@10.
Compared with CodeGen, which is pre-trained with a fixed size of context (the \emph{m} nearest tokens before the function to be generated, \emph{m} is the window size), \wenwangcoder{} is fine-tuned with a broader scope of context by extracting contextual information via program analysis, so it is able to consume more context more efficiently, especially under the limited window size 1024 of the 300M models.


Given the oracle\_context and the docstring, the four models all perform better than given the docstring only. 
The preceding result indicates that providing the correct or expected contextual information to use is a reliable way to improve the accuracy of code generation.
By manually inspecting the generated code when prompting with and without the oracle\_context, we find that the model does show a tendency to use the provided contextual to fulfill the expected function, which also conforms to common sense.
However, while \wenwangcoder{} achieves the highest Pass@1 value, it falls behind CodeGen, \codePLM{}, and PanGu-FT at Pass@5 and Pass@10.
We consider this phenomenon explainable: On one hand, directly providing the oracle context does help the model to generate correct solutions in an expected way, but on the other hand, it also restricts the solution space of the model and the diversity of the generated code. Since the Pass@K metric evaluates the behavior correctness, it does not require the correct solution to be exactly the same, so providing the all\_context and letting the model choose by itself may result in higher Pass@K values.





% ----TO ADD----
% On one hand, providing the oracle context directly does help the model to generate correct solutions, comparing with providing the docstring only. But on another hand, it also restricts the solution space of the model. Since the Pass@K metric based on behavior corretness does not require the exactly same solution, providing the all context alongside docstring and letting the model choose what to use results in higher Pass@K values, which holds for K=1, 5 and 10.
% Based on this observation, we anticipate that by integrating API recommendation tools [] to provide possibly-used APIs as the context will further improve the model's performance, which is part of our future work on context-aware code generation.
% Although Wenwang may benefit from the fine-tuning process, given other input formats, it still outperforms or on par with the other 2 models


==> evaluation/rq3.tex <==
% \subsection{RQ4: How do \codePLM{}, CodeGen, and \wenwangcoder{} perform on \wenwangbench{} excludes the functions with none return type?}

% \begin{table}[t]
%     \centering
%     \footnotesize	
%     \caption{RQ4: Performance of 3 Models Across 6 Runnable Levels only on functions with return values}
%     \vspace*{-1.5ex}
%     \label{tab: multi performance on wenwangbench excludes none return type}
%     \begin{tabular}{@{}rcrrrrrrrr@{}} 
%         \midrule
%         Runnable Level &  \multicolumn{1}{c}{Model}  & pass@1 & pass@5 & pass@10\\
%         \midrule
%         \multirow{3}{*}{self\_contained} &  CodeGen  &  17.14\% & 34.82\% & 37.14\% \\
%         & \codePLM{} & 21.14\% &34.92\% & 40.00\% \\
%         & \wenwangcoder{} & \textbf{28.00\%} & \textbf{39.85\%} & \textbf{42.86\%} \\
%         \midrule
%         \multirow{3}{*}{slib\_runnable} &  CodeGen  & 8.21\% & 20.04\% & 25.00\% \\
%         & \codePLM{} &  \textbf{12.50\%} & \textbf{24.89\%} & \textbf{32.14\%} \\
%         & \wenwangcoder{} & 12.14\% & 20.55\% & 25.00\% \\
%         \midrule
%         \multirow{3}{*}{plib\_runnable} & CodeGen & 6.84\% & 20.36\% & 26.32\% \\
%         & \codePLM{} & \textbf{13.16\%} & \textbf{25.13\%} & \textbf{31.58\%} \\
%         & \wenwangcoder{} & 11.05\% & 18.30\% & 21.05\% \\
%         \midrule
%         \multirow{3}{*}{class\_runnable} & CodeGen & 8.89\% & 14.66\% & 16.67\% \\
%         & \codePLM{} & 11.39\% & 12.50\% & 13.89\% \\
%         & \wenwangcoder{} & \textbf{13.61\%} & \textbf{17.92\%} & \textbf{19.44\%} \\
%         \midrule
%         \multirow{3}{*}{file\_runnable} & CodeGen &  7.64\% & 14.45\% & 16.36\% \\
%                 & \codePLM{} & 10.36\% & 13.23\% & 14.55\% \\
%         & \wenwangcoder{} & \textbf{10.73\%} & \textbf{16.42\%} & \textbf{20.00\%} \\
%         \midrule
%         \multirow{3}{*}{project\_runnable} & CodeGen & 0\% & 0\% & 0\% \\
%         & \codePLM{} & 0\% & 0\% & 0\% \\
%         & \wenwangcoder{} & 0\% & 0\% & 0\% \\
%         \midrule
%         \multirow{3}{*}{over\_all} & CodeGen & 8.85\% & 18.17\% & 20.83\% \\
%         & \codePLM{} & 12.08\% & 18.62\% & 21.88\% \\
%         & \wenwangcoder{} & \textbf{13.59\%} & \textbf{20.14\%} &  \textbf{22.92\%} \\
%         \bottomrule
%     \end{tabular}
%     \vspace*{-2.5ex}
% \end{table} 


% In the previous sections, we discussed and analyzed the overall and six runnable levels performance of CodeGen, \codePLM{}, and \wenwangcoder{} on \wenwangbench{}. 
% To further analyze \wenwangbench{}, this section describes in detail the proportion of functions with none return value in \wenwangbench{} and the experimental results after removing these functions in \wenwangbench{}.
% In realistic development scenarios, many functions do not have return values. 
% Since \wenwangbench{} is built from open-source projects, some functions do not have return values. For these functions with none return value, we do not think it is correct to force a return value to them, because the model can also generate many functions with none return value. So we keep these functions in \wenwangbench{}, and in the previous experiments, we considered them correct as long as the code generated by models for these functions with none return value had a return value of none and had no error in the code execution. 
% This ensures that we may miss the wrong program, but not the right one.
% In addition, we know that this may affect the model effect. Therefore, in this section, we remove the functions whose return value is None from the benchmark and then test the effects of the three models on the benchmark. The experimental results show that the overall performance of \wenwangcoder{} is also higher than that of CodeGen and \codePLM{} after removing the functions whose return value is None.

% \subsubsection{Overall and six runnable levels performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} excludes the functions with none return type}


% Table~\ref{tab: multi performance on wenwangbench excludes none return type} shows the overall and six runnable levels performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} excludes the functions with none return type.
% From the last raw in the table, we can observe that \wenwangcoder{} also outperforms \codePLM{} and CodeGen on all pass@ks. 
% Compared with Table~\ref{tab: overall performance for wenwangbench and he}, after excluding the functions with none return type in \wenwangbench{}, all models have a slight decrease in effectiveness.




\subsection{RQ3: How does the performance of different models vary on the original and human-labeled docstrings in \wenwangbench{}?}

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2pt}
    \caption{Performance with 2 Prompt Versions of \wenwangbench}
    \vspace*{-1.5ex}
    \label{tab: overall performance for wenwangbench with human label}
    \begin{tabular}{@{} crc|ccccc @{}} % suppress vertical whitespace at start and end
        \toprule
        \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Prompt}} & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
        \cmidrule(lr){3-6}
        &  &  pass@1(greedy) & pass@1 & pass@5 & pass@10\\
        \midrule
        \multirow{2}{*}{CodeGen} &  Original &  10.87\%  &  9.26\% & 21.29\% & 25.22\% \\
        & Human Label &  11.30\%   & 11.91\% & 23.34\% & 26.52\% \\
        \midrule
        \multirow{2}{*}{\codePLM} &  Original  & 13.04\%   & 11.96\% & 19.73\% & 23.91\%  \\
        & Human Label &  15.22\%  & 14.22\% &21.74\% & 25.22\% \\
        \midrule
        \multirow{2}{*}{PanGu-FT} &  Original  & 13.48\%   & 13.09\% & 19.80\% & 22.61\% \\
        & Human Label &  15.65\%   & 15.35\% & 22.96\% & 26.09\% \\
        \midrule
        \multirow{2}{*}{\wenwangcoder} &  Original  & 16.09\%   & 14.43\% & 22.29\% & 25.65\% \\
        & Human Label &  17.83\%   & 16.70\% & 23.93\% & 26.96\% \\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
\end{table} 
Besides the original docstring, each function in CoderEval also has human\_labeled docstring.
To explore the impact of prompts with human labeling on the code generated by large language models, we conduct experiments for different models with an original docstring and human\_labeled docstring on CoderEval.
% During the research and case study, we find that the quality of original docstrings from the open-source projects is rather unstable and inconsistent, so we wonder if they are a good choice as the prompt for code generation models.
% In practice, the function-level docstring or comment can play several different roles: explaining the internal logic, introducing the external usage and behavior, declaring the effect and caution, etc.
% Therefore, docstrings can be at different abstract levels and granularity. 
% The quality of docstring can have a great impact on the quality of generated code.
% Existing study~\cite{Sarkar2022prompt} shows the prompts are important for large language models, and writing effect prompts is difficult. Therefore, this paper also tries to explore the impact of prompts with human labeling on the quality of code generated by large language models.
% Codex removes problems with ambiguous descriptions by trying to generate with the pre-trained model, but we decide to face the fact and additionally provide a human-labeled version of docstring for each problem in \wenwangbench{}, which is labeled by 13 software engineers with at least 3-year experience of Python through a two-fold cross-validation process.

% \subsubsection{Performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{} with the original and human-labeled docstring}

\begin{figure}
\centering
\subfigure[\wenwangcoder{} with pre-trained models ]{
\label{fig.complenmenthlpretrain}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{figure/hlpretraincom.pdf}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[\wenwangcoder{} with fine-tuned models ]{
\label{fig.complenmenthlfinetune}
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{figure/hlfinetunecom.pdf}
\end{minipage}%
}%
\centering
\caption{Number of functions that models fail to solve with the original docstring but succeed with the human-labeled version}
\label{fig.complenment_humanlabel}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.5\linewidth]{figure/complementarity-humancorrect.pdf}
% 	\caption{The number of functions that models fail to solve with the original docstring but succeed with the human-labeled version}
% 	\label{fig.complenment_humanlabel}
%  \vspace*{-1ex}
% \end{figure}


We evaluate the different models on both the original and the human-labeled docstring and show the result in Table~\ref{tab: overall performance for wenwangbench with human label}.
Overall, compared with the original docstring, the human-labeled version does bring improvements to all models.
Although the original docstring was written by the original code author, some of them are too simple and abstract, underspecifying the logic and intent of the function.
On the contrary, the human-labeled docstring was written by the participants after careful consideration and understanding of the entire project, so it tends to be more specific and concentrated, which is beneficial for the model to understand the intent.


% Table~\ref{tab: overall performance for wenwangbench} shows the overall performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{}. 
% As shown in the table, we find that when n is 10, whether k is 1, 5, or 10, \wenwangcoder{} is significantly better than \codePLM{} and CodeGen. Especially when k is 1, the effect of \wenwangcoder{} is much higher than that of \codePLM{} and CodeGen.


Figure~\ref{fig.complenmenthlpretrain} shows the number of functions that are incorrectly generated by the original docstring, but correctly generated by the human-labeled docstring for CodeGen, \codePLM{}, and \wenwangcoder{}.
Similar to Section~\ref{sec:comall}, we also consider a problem to be solved if the model can generate \emph{at least} one correct solution that passes all tests out of the ten generated solutions.
Overall, the total number of functions that are solved by only changing the docstring for the three models is 26, but interestingly, their intersection is only 1.
Figure ~\ref{fig.complenmenthlfinetune} shows a similar phenomenon to Figure ~\ref{fig.complenmenthlpretrain}. 
% Figure~\ref{fig.complenmenthlfinetune} shows the number of functions that are correctly generated when replacing the original docstring with the human-labeled version for WWDocs, PanGu-FT, and \wenwangcoder{}.
% The total number of problems that are solved by only changing the docstring for the three models is 25, but interestingly, their intersection is only 3.
Experimental result indicates different models' (neither pre-trained nor fine-tuned) are highly sensitive to the prompt, as well as the high complementarity in their capability.


Figure~\ref{fig.case_humanlabel} shows an example of a function in \wenwangbench{}, with the two versions of docstrings and two solutions generated by \wenwangcoder{}.
The task is to remove and return the first enqueued element from the data object.
The left part shows the original docstring and an incorrect solution, which is incorrect because the generated code returns the last element instead of the first and does not remove it before returning.
The right part shows the human-labeled docstring that details the expected behavior of the function and a correct solution that is different but equivalent to the original code.
% Due to the page limitation, we leave more examples in the supplementary appendix.
\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{figure/HumanLabel_case_study.pdf}
	\caption{An example of the functions incorrectly generated with the original docstring but correctly generated with the human-labeled docstring}
	\label{fig.case_humanlabel}
  \vspace*{-1ex}
\end{figure}



% We anticipate that the problem also exist in the pre-training dataset, The large language model is very sensitive to the prompt and more research work can be done in guiding the user to provide a proper docstring

==> evaluation/rq3_back.tex <==
\subsection{RQ3: How does the performance of four models correctly utilise the contextual information? }

\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2pt}
    \caption{RQ3: The accuracy of three models that they can correctly generate the contextual tokens}
    \vskip 0.15in
    \label{tab: contextual}
    \begin{tabular}{@{} cc|cccccccc @{}} % suppress vertical whitespace at start and end
        \toprule
        % \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Prompt}} 
        % & & \multicolumn{4}{c}{Python} & \multicolumn{4}{c}{Java} &
        \multicolumn{1}{c}{\multirow{2.5}{*}{Model}} & \multicolumn{1}{c}{\multirow{2.5}{*}{Contextual Type}}  & \multicolumn{4}{c}{Acc@K}\\
        \cmidrule(lr){3-6} 
        % & & \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}& \multicolumn{1}{c|}{n=1} & \multicolumn{3}{c}{n=10}\\
        %  \cmidrule(lr){4-6}  \cmidrule(lr){8-10}
         & & Average& Acc@1 & Acc@5 & Acc@10\\
        \midrule
        \multirow{3}{*}{CodeGen} &  TypeReference  &  12.63\%&  13.01\% &  22.97\% & 25.93\% \\
        & APIInvocation   &  7.78\%&  7.04\%& 17.40\% & 21.90\%\\
        & VarReference   & 3.37\% & 3.45\% & 7.10\% &8.36\%\\
        \midrule
        \multirow{3}{*}{\codePLM} &  TypeReference  & 13.16\%&11.06\%&  22.80\% & 26.46\% \\
        & APIInvocation   & 6.64\%&5.95\%& 11.22\% & 14.53\% \\
        & VarReference  &3.15\%& 3.08\%& 4.60\% & 5.30\% \\
        \midrule
        \multirow{3}{*}{\wenwangcoder{}} &  TypeReference   & 19.98\%&21.54\%&  31.01\% & 34.48\% \\
        & APIInvocation   & 12.51\%&10.99\%&23.71\% &29.76\%\\
        & VarReference   & 4.12\%&4.20\%& 8.86\% & 11.04\%\\
        \bottomrule
    \end{tabular}
    \vspace*{-2.5ex}
    
\end{table} 

To further study the \emph{context-awareness} of large language models, we analyze the identifier tokens in generated code and focus on three types of tokens: TypeReference, APIInvocation, and VarReference (including constants reference).
Table~\ref{tab: contextual} shows the Acc@k of three models, we find it is consistent with Pass@K (i.e., the generated functions can pass test cases), and the Acc@K of Codex is also the best one in generating contextual dependency. 
To further explore the ability of different models in generating different types of context information, we divide the context token into three categories: TypeReference, APIInvocation, and VarReference, which usually form the most important part of the implementation at runnable-levels with external dependency.
%We do not classify constants because, in common programming habits, developers often use a global variable declaration for a constant, which is context-dependent. 
As shown in Table~\ref{tab: contextual}, on \wenwangbench{}, all models show poor effectiveness in generating the correct ``VarReference'' token, while the effectiveness in generating ``TypeReference'' token is relatively good.

Compared with \codePLM{} and CodeGen, \wenwangcoder{} performance best in correctly utilizing the contextual information.


% Table~\ref{tab: overall performance for wenwangbench} shows the overall performance of \codePLM{}, CodeGen, and \wenwangcoder{} on \wenwangbench{}. 
% As shown in the table, we find that when n is 10, whether k is 1, 5, or 10, \wenwangcoder{} is significantly better than \codePLM{} and CodeGen. Especially when k is 1, the effect of \wenwangcoder{} is much higher than that of \codePLM{} and CodeGen.


% Figure~\ref{fig.complenment_humanlabel} shows the number of functions that are correctly generated when replacing the original docstring with the human-labeled version.
% Overall, for all three models, the number of problems that are solved by only changing the docstring is 11, but interestingly, their intersection is only 1.
% This indicates different models' sensitivity to the prompt, as well as the complementarity in their capability.


% Figure~\ref{fig.case_humanlabel} shows an example function in \wenwangbench{}, with the two versions of docstrings and two solutions generated by \wenwangcoder{}.
% The task is to remove and return the first enqueued element from the data object.
% The left part shows the original docstring and an incorrect solution, which is incorrect because the generated code returns the last element instead of the first and does not remove it before returning.
% The right part shows the human-labeled docstring that details the expected behavior of the function and a correct solution that is different but equivalent to the original code.
% Due to the page limitation, we leave more examples in the supplementary appendix.
% \begin{figure}
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figure/HumanLabel_case_study.pdf}
% 	\caption{An example of the functions incorrectly generated with the original docstring but correctly generated with the human-labeled docstring}
% 	\label{fig.case_humanlabel}
%   \vspace*{-1ex}
% \end{figure}



% % We anticipate that the problem also exist in the pre-training dataset, The large language model is very sensitive to the prompt and more research work can be done in guiding the user to provide a proper docstring
